Wastewater-based Epidemiology for COVID-19 Surveillance and Beyond: A Survey

The pandemic of COVID-19 has imposed tremendous pressure on public health systems and social economic ecosystems over the past years. To alleviate its social impact, it is important to proactively track the prevalence of COVID-19 within communities. The traditional way to estimate the disease prevalence is to estimate from reported clinical test data or surveys. However, the coverage of clinical tests is often limited and the tests can be labor-intensive, requires reliable and timely results, and consistent diagnostic and reporting criteria. Recent studies revealed that patients who are diagnosed with COVID-19 often undergo fecal shedding of SARS-CoV-2 virus into wastewater, which makes wastewater-based epidemiology for COVID-19 surveillance a promising approach to complement traditional clinical testing. In this paper, we survey the existing literature regarding wastewater-based epidemiology for COVID-19 surveillance and summarize the current advances in the area. Specifically, we have covered the key aspects of wastewater sampling, sample testing, and presented a comprehensive and organized summary of wastewater data analytical methods. Finally, we provide the open challenges on current wastewater-based COVID-19 surveillance studies, aiming to encourage new ideas to advance the development of effective wastewater-based surveillance systems for general infectious diseases.

==> glossary.tex <==
% 暂时废弃
\makeglossaries

\newglossaryentry{WBE}{
    name={WBE},
    description={Wastewater-Based Epidemiology}
}

\newglossaryentry{WWTPs}{
    name={WWTPs},
    description={WasteWater Treatment Plants}
}

\newglossaryentry{PRISMA}{
    name={PRISMA},
    description={Preferred Reporting Items for Systematic Reviews and Meta-Analyses}
}


\newglossaryentry{SLR}{
    name={SLR},
    description={Systematic Literature Review}
}

\newglossaryentry{NWSS}{
    name={NWSS},
    description={National Wastewater Surveillance System}
}


\newglossaryentry{PEG}{
    name={PEG},
    description={Polyethylene Glycol}
}


\newglossaryentry{PCR}{
    name={PCR},
    description={Polymerase Chain Reaction}
}


\newglossaryentry{RT-LAMP}{
    name={RT-LAMP},
    description={Reverse
Transcription Loop-mediated Isothermal Amplification}
}


\newglossaryentry{RT-qPCR}{
    name={RT-qPCR},
    description={Reverse Transcription-quantitative Polymerase Chain Reaction}
}

\newglossaryentry{RT-ddPCR}{
    name={RT-ddPCR},
    description={RT-droplet Digital PCR}
}


\newglossaryentry{PMMoV}{
    name={PMMoV},
    description={Pepper Mild Mottle virus}
}


\newglossaryentry{QC}{
    name={QC},
    description={Quality Control}
}


\newglossaryentry{QA}{
    name={QA},
    description={Quality Assurance}
}


\newglossaryentry{WRF}{
    name={WRF},
    description={Water Research Foundation}
}


\newglossaryentry{CrI}{
    name={CrI},
    description={Credible Interval}
}

\newglossaryentry{SEIR-model}{
    name={SEIR model},
    description={Susceptible Exposed Infectious Recovered \\model}
}

\newglossaryentry{POMP}{
    name={POMP},
    description={Partially Observed Markov Processes model }
}


\newglossaryentry{EKF}{
    name={EKF},
    description={Extended Kalman Filter}
}

\newglossaryentry{ARIMA}{
    name={ARIMA},
    description={AutoRegressive Integrated Moving Average}
}

\newglossaryentry{RMSE}{
    name={RMSE},
    description={Root Mean Squared Error}
}


\newglossaryentry{VAR}{
    name={VAR},
    description={Vector Autoregression}
}


\newglossaryentry{MAPE}{
    name={MAPE},
    description={Mean Average Percentage Error}
}


\newglossaryentry{SARIMA}{
    name={SARIMA},
    description={AutoRegression Model with Seasonal Patterns}
}

\newglossaryentry{LSOAs}{
    name={LSOAs},
    description={Lower Super Output Areas}
}


\newglossaryentry{LTLA}{
    name={LTLA},
    description={Lower Tier Local Authority}
}

\newglossaryentry{LR}{
    name={LR},
    description={Linear Regression}
}

\newglossaryentry{PL}{
    name={PL},
    description={Polynomial Regression}
}

\newglossaryentry{KNN}{
    name={KNN},
    description={$k$ Nearest Neighbor}
}

\newglossaryentry{MLP}{
    name={MLP},
    description={Multilayer Perceptron}
}

\newglossaryentry{SVR}{
    name={MLP},
    description={Support Vector Regression}
}

\newglossaryentry{GAM}{
    name={GAM},
    description={Generalized Additive Models}
}

\newglossaryentry{DT}{
    name={DT},
    description={Decision Tree}
}

\newglossaryentry{RF}{
    name={RF},
    description={Random Forest}
}

\newglossaryentry{LOESS}{
    name={LOESS},
    description={Locally Estimated Scatterplot Smoothing \\model}
}


\newglossaryentry{GBRT}{
    name={GBRT},
    description={Gradient Boosted Regression Trees}
}

\newglossaryentry{ANN}{
    name={ANN},
    description={Artificial Neural Network model}
}

\newglossaryentry{ANFIS}{
    name={ANFIS},
    description={Adaptive Neuro Fuzzy Inference System }
}

\newglossaryentry{WC-ratio}{
    name={WC ratio},
    description={the Ratio between Wastewater Viral Load and Clinical Cases}
}









